Harnessing Scale and Physics: A Multi-Graph Neural Operator Framework for PDEs on Arbitrary Geometries

Partial Differential Equations (PDEs) underpin many scientific phenomena, yet traditional computational approaches often struggle with complex, nonlinear systems and irregular geometries. This paper introduces the AMG method, a Multi-Graph neural operator approach designed for efficiently solving PDEs on Arbitrary geometries. AMG leverages advanced graph-based techniques and dynamic attention mechanisms within a novel GraphFormer architecture, enabling precise management of diverse spatial domains and complex data interdependencies. By constructing multi-scale graphs to handle variable feature frequencies and a physics graph to encapsulate inherent physical properties, AMG significantly outperforms previous methods, which are typically limited to uniform grids. We present a comprehensive evaluation of AMG across six benchmarks, demonstrating its consistent superiority over existing state-of-the-art models. Our findings highlight the transformative potential of tailored graph neural operators in surmounting the challenges faced by conventional PDE solvers. Our code and datasets are available on https://github.com/lizhihao2022/AMG.

==> tables/config.tex <==
\begin{table*}[ht]
\vspace{-10pt}
\centering
\caption{Details of hyperparameters used for benchmarks.}
\label{table:config}
\renewcommand\arraystretch{0.8}
\begin{sc}
    \renewcommand{\multirowsetup}{\centering}
    \vspace{-5pt}
    % \setlength{\tabcolsep}{4.7pt}
    \resizebox{0.98\linewidth}{!}{
    \begin{tabular}{c|cccccc}
       \toprule
       Type & NS & Shape-Net Car & Poisson & Cylinder Flow & DP & Airfoil \\
       \midrule
        input\_features  & 1    & 4    & 1    & 3    & 1    & 4    \\
        output\_features & 1    & 4    & 1    & 3    & 1    & 4    \\
        feature\_width   & 128  & 128  & 128  & 128  & 128  & 128  \\
        pos\_dim         & 2    & 3    & 2    & 2    & 3    & 2    \\
        num\_layers      & 3    & 3    & 3    & 3    & 2    & 3    \\
        activation          & 'relu'        & 'relu'        & 'relu'  & 'relu'        & 'relu'          & 'relu'  \\
        batch\_norm      & TRUE & TRUE & TRUE & TRUE & TRUE & TRUE \\
        global\_ratio    & 0.25 & 0.25 & 0.25 & 0.25 & 0.1  & 0.25    \\
        global\_k        & 4    & 4    & 4    & 4    & 3    & 4    \\
        local\_nodes     & 1024 & 512  & 512  & 1024 & 128  & 512  \\
        local\_k         & 6    & 6    & 6    & 6    & 6    & 6    \\
        num\_phys        & 32   & 32   & 32   & 32   & 32   & 32   \\
        num\_heads       & 8    & 8    & 8    & 8    & 8    & 8   \\
       \bottomrule
    \end{tabular}}
\end{sc}
\vspace{-5pt}
\end{table*}
